Branching Fractions and CP-Violating Asymmetries in Radiative B Decays to eta K gamma

We present measurements of the CP-violation parameters S and C for the radiative decay B0 -> eta K0s gamma; for B -> eta K gamma we also measure the branching fractions and for B+ -> eta K+ gamma the time-integrated charge asymmetry Ach. The data, collected with the BaBar detector at the Stanford Linear Accelerator Center, represent $465 \times 10^6$ BBbar pairs produced in $e^{+} e^{-}$ annihilation. The results are $S = -0.18^{+0.49}_{-0.46} \pm 0.12$, $C = -0.32^{+0.40}_{-0.39} \pm 0.07$, BF(B0 -> eta K0 gamma) = $(7.1^{+2.1}_{-2.0} \pm 0.4) \times 10^{-6}$, BF(B+ -> eta K+ gamma) = $(7.7+-1.0 \pm 0.4) \times 10^{-6}$, and Ach = $(-9.0^{+10.4}_{-9.8} \pm 1.4) \times 10^{-2}$. The first error quoted is statistical and the second systematic.

==> abstract.tex <==
We present  measurements of the CP-violation parameters
$S$ and $C$ for the radiative decay $B^0 \rightarrow \eta \K^0_s
\gamma$; for $B \rightarrow \eta K \gamma$ we also measure the
branching fractions and for $B^+ -> \eta K^+ \gamma$ the
time-integrated charge asymmetry $A_{ch}$. 
The data, collected with the BaBar detector at the Stanford Linear
Accelerator Center, represent $465 \times 10^6$ $B \bar{B}$ pairs
produced in 
$e^+ e^-$ annihilation. The results are $S = -0.18^{+0.49}_{-0.46} \pm
0.12$, $C = -0.32^{+0.40}_{-0.39} \pm 0.07$, ${\cal B} (B^0
\rightarrow \eta \K^0 \gamma) = (7.1^{+2.1}_{-2.0} \pm 0.4) \times
10^{-6}$, ${\cal B} (B^+ \rightarrow \eta \K^+ \gamma) = 
(7.7+-1.0 \pm 0.4)  \times 10^{-6}$, and $A_{ch} = (-9.0^{+10.4}_{-9.8}
\pm 1.4) \times 10^{-2}$.
The first error quoted is statistical and the second systematic.

